In-Hand Gravitational Pivoting Using Tactile Sensing

We study gravitational pivoting, a constrained version of in-hand manipulation, where we aim to control the rotation of an object around the grip point of a parallel gripper. To achieve this, instead of controlling the gripper to avoid slip, we embrace slip to allow the object to rotate in-hand. We collect two real-world datasets, a static tracking dataset and a controller-in-the loop dataset, both annotated with object angle and angular velocity labels. Both datasets contain force-based tactile information on ten different household objects. We train an LSTM model to predict the angular position and velocity of the held object from purely tactile data. We integrate this model with a controller that opens and closes the gripper allowing the object to rotate to desired relative angles. We conduct real-world experiments where the robot is tasked to achieve a relative target angle. We show that our approach outperforms a sliding-window based MLP in a zero-shot generalization setting with unseen objects. Furthermore, we show a 16.6% improvement in performance when the LSTM model is fine-tuned on a small set of data collected with both the LSTM model and the controller in-the-loop. Code and videos are available at https://rhys-newbury.github.io/projects/pivoting/

==> old_text.tex <==
% old intro (might take some from here later)



In-hand manipulation, which involves re-orientation and re-positioning of held objects, is a fundamental skill required for complex handling of real-world objects. For robots, a strong capability to manipulate objects is required for general purpose interaction with the real world~\cite{4141029}. Such manipulation capability is trivial for humans, as we can use information gathered from multiple sources, such as visual, tactile, audio as well as past experiences. We can then use this complex information to control our fingers simultaneously to precisely re-orient an object, sometimes even using features of the environment and taking advantage of our intuitive understanding of physics. Even though there have been recent successful demonstrations of robotic systems capable of in-hand manipulation \cite{openai2019learning, chen2021system}, several challenges remain, including compliant mechanical design, and robust control algorithms that use multi-modal sensing including visual, touch and force~\cite{billard2019trends}. 

Robotic in-hand manipulation is almost always implemented with robotic hands, because the high DOF gives opportunity to mimic the capabilities of the human hand. However, today's robotic hands are still a poor proxy for the human hand because they are composed of rigid components with electric motors as actuators~\cite{billard2019trends}. Also, such robotic hands are not as common as simpler grippers such as  parallel grippers. Due to the prevalence of such simple grippers, developing in-hand manipulation strategies for parallel grippers is crucial to expand the capabilities of simple robots.

With parallel grippers, it is often assumed that the object does not move after it has been grasped, but in reality, it is common for the object to move. This movement could be caused by slip due to weak grasps, external pushes against the object etc. Although the most common approaches are to simply detect slip and prevent its occurrence, slip can also be utilised to perform in-hand manipulation. This is especially helpful for parallel grippers due to their significant limitation in motion. Hence, to improve the manipulation skills of robots with simple parallel grippers, we explore novel methods of inducing and exploiting rotational slip for manipulation tasks. Instead of pushing against obstacles in the environment to perform in-hand manipulation~\cite{chavandafle2017samplingbased}, we propose adjusting the grip strength and utilizing gravitational forces.

Hence, this paper proposes a method to allow for a robot with a parallel gripper to rotate an arbitrary, long object grasped away from it's center of mass to a desired final orientation required for some later task using only gravity. This will allow for parallel grippers to robustly reorient objects into a desired orientation without having to grasp, place and regrasp the object.



We propose 2 contributions:

\textbf{Rotational Slip Quantitative Estimation}: A deep learning method to measure the rotation of an object held by the robot purely though tactile feedback. This will use models such as the long short-term memory (LSTM) model \cite{articleLSTM} and the Transformer \cite{vaswani2017attention}, with tactile sensor data as inputs.

\textbf{Grip Controller}: A controller to loosen the robot's grip, to allow a held object to rotationally slip using gravitational force. The object will then rotate until either a desired final orientation is achieved or the object comes into contact with the ground. The controller will then maintain a loose grip so that the object can maintain it's orientation while the end effector moves and rotates.

We propose evaluating our solutions on 2 tasks:

\begin{itemize}
\item \textbf{Wine bottle reorientation:} Grasping a wine bottle and rotating it such that it is parallel with the gripper and can be inserted into a wine rack easily.
\item \textbf{Droop\&drag manipulation:} Allowing an object to freely rotate so it can be dragged into a desired position along a planar surface, as in \cite{2021droop}.
\end{itemize}




\section{Proposed Approach}

Our approach consists of two main components. A Rotational Slip Estimator LSTM (RSE-LSTM) and a Grip Controller.

From purely tactile information, the RSE-LSTM will estimate the angle between the principle axis (long axis) of the object and the vertical-z axis. The Grip Controller will use the angle estimation and gravitational pivoting to allow the object to reach arbitrary angles. 

\subsection{Rotational Slip Estimator}

The RSE-LSTM will take force measurements from the tactile sensors as inputs, and predict the current angular velocity of the object as the output. This angular velocity can then be integrated to give the rotation of the object from its starting angle. It is assumed that the initial rotation of the object is known, so this measurement will be enough information to determine the orientation of the object in space.

The RSE-LSTM model will consist of an LSTM, the outputs of which are passed to a MLP. The model will run at 60 Hz due to hardware limitations in training data collection. While training the model, data will be batched by cropping sequences to be the same length as the shortest sequence in the batch.
% TODO
% Network Diagram

\subsection{Grip Controller}
% Simple heuristics will be used to allow for the controller to be easily generalised to any object. As in the approach to rotation estimation, the gripper will pick up the object from a vertical orientation.

It is assumed that initially an object is held by the parallel gripper away from its center of mass. The gripper will then be slowly opened incrementally until rotation is detected. The object will then be allowed to rotate. If the object is recorded to have achieved a fully vertical orientation the grip will be tightened to allow for movement of the object without further slip occurring. If the object is not yet fully vertical, the gripper is again loosened until a fully vertical orientation is achieved. Once a fully vertical orientation has been achieved, the end effector will rotate to achieve an arbitrary final orientation while allowing the object to slip and maintain it's fully vertical orientation. An alternate outcome is that the object hits the ground as it is rotating. To detect this outcome, a shallow MLP will be trained that takes 2 inputs:
\begin{itemize}
    \item The initial sensor values before the object was released. 
    \item The current sensor values
\end{itemize}
The MLP will then perform a binary classification to determine if the object is resting on the ground.



==> system_diagram.tex <==
\begin{tikzpicture}
 
% Sum shape
% \node[draw,
%     circle,
%     minimum size=0.6cm,
%     fill=Rhodamine!50
% ] (sum) at (0,0){};
 
%  \tikzstyle{every node}=[]

 
\node[draw, 
      thin,
      draw=black,
      ellipse,
      minimum width=2cm,
      minimum height=1cm,
      align=center,
      fill=SpringGreen] (lstm) at (0,0) {RSE-LSTM};

% Controller
\node [draw,
    fill=SpringGreen,
    minimum width=2cm,
    thin,
    draw=black,
    ellipse,
    minimum width=2cm,
    minimum height=1cm,
    align=center,
    minimum height=1.2cm,
    right=2.5cm of lstm
]  (controller) {Grip Controller};

% Controller
\node [draw,
    fill=SpringGreen,
    minimum width=2cm,
    thin,
    draw=black,
    ellipse,
    minimum width=2cm,
    minimum height=1cm,
    align=center,
    minimum height=1.2cm,
    right=2.5cm of controller
]  (gripper) {Parallel Jaw Gripper};


% Controller
\node [draw,
    fill=SpringGreen,
    minimum width=2cm,
    thin,
    draw=black,
    ellipse,
    minimum width=2cm,
    minimum height=1cm,
    align=center,
    minimum height=1.2cm,
    below=2.5cm of controller
]  (sensor) {Tactile Sensor};

 
% % Sensor block
% \node [draw,
%     fill=Goldenrod, 
%     thin,
%     draw=black,
%     ellipse,
%     minimum width=2cm,
%     minimum height=1cm,
%     align=center,
%     below= 1.5cm of camera
% ]  (od) {Object\\Detection};


% \node [draw,
%     fill=Goldenrod, 
%     thin,
%     draw=black,
%     ellipse,
%     minimum width=2cm,
%     minimum height=1cm,
%     align=center,
%     right= 2cm of od
% ]  (gs) {Grasp\\Selection};

% \node [draw,
%     fill=Goldenrod, 
%     thin,
%     draw=black,
%     ellipse,
%     minimum width=2cm,
%     minimum height=1cm,
%     align=center,
%     right= 2cm of gs
% ]  (mc) {Robot Motion \\ Control};


% \node [draw,
%     fill=SpringGreen, 
%     thin,
%     draw=black,
%     ellipse,
%     minimum width=2cm,
%     minimum height=1cm,
%     align=center,
%     right= 2cm of mc
% ]  (ra) {Robot Arm};

 
% % Arrows with text label
% \draw[-latex] (camera.south) -- (od.north)
%     node[midway,left]{RGB-D Image};
    
% \draw[-latex] (od.east) -- (gs.west)
%     node[midway,below]{Object Pose};
 
% %  \draw[-latex] (od.east)+(0,0.5mm) |- (hololens.west)
% %     node[midway,left]{Object Wireframe};

% \draw [-latex] (od.east)++(-0.03,0.2) --  node[anchor=east, above=2pt ]{} ++(1.25,0) |- (hololens.west)node[above,at start, align=center, anchor=south west, yshift=75pt, xshift=0pt]{Object\\Wireframe};
 
% \draw [-latex] (gs.north) --  node[anchor=east, above=2pt ]{} ++(0,1) -| (hololens.south)node[above,at start, align=center, anchor=south west, yshift=-15pt]{Grasp Point};
 
 
% % \draw[-latex] (gs.north) -- (hololens.south)
% %     node[midway,left]{Grasp Point};
    
% \draw[-latex] (gs.east) -- (mc.west)
%     node[midway,above]{Grasp Point};
    
%  \draw[-latex] (hololens.east) -| (mc.north)
%     node[midway,right]{Voice Command};
 
%  \draw[-latex] (mc.east) -- (ra.west)
%     node[midway,below]{Joint Velocity};


% \begin{document}?
% \begin{tikzpicture}
%   \node[entity] (od) {Object Detection};
%   \node[entity] (gs) {Grasp Selection};
%   \node[entity] (mc) {Robot Motion Control};
    
%   \node[attribute] (pid) [left = of person] {\key{ID}} edge (person);
%   \node[attribute] (name) [above left = of person] {Name} edge (person);
% \end{tikzpicture}
% \end{document} 
 
% \draw[-stealth] (hololens.east) -- (system.west) 
%     node[midway,above]{$u$};
 
% \draw[-stealth] (system.east) -- ++ (1.25,0) 
%     node[midway](output){}node[midway,above]{$y$};
 
% \draw[-stealth] (output.center) |- (sensor.east);
 
% \draw[-stealth] (sensor.west) -| (sum.south) 
%     node[near end,left]{$y_m$};
 
% \draw (sum.west) -- ++(-1,0) 
%     node[midway,above]{$y_{ref}$};
 
 
\end{tikzpicture}
 
